Robust Error Bounds for Vector-Valued Kernel Ridge Regression

While kernel-based learning methods for scalar-valued functions have been extensively studied, comparatively little work considers nonlinear vector-valued operators. Such operators with vector-valued outputs, e.g., state vectors and trajectories, commonly arise in system identification problems. In this paper, we study the problem of learning a vector-valued operator under the framework of vector-valued kernel ridge regression. We assume that the outputs take values in an arbitrary Hilbert space and are corrupted by additive noise with bounded norm. Under the assumption that the unknown operator belongs to a vector-valued reproducing kernel Hilbert space, we derive a pointwise deterministic bound on the discrepancy between the kernel ridge regression estimator and the ground truth in the corresponding Hilbert space norm. Numerical simulations under two different scenarios are presented to validate the theoretical results.

==> section/4_efficient_computation.tex <==
\section{Efficient computation}

% For instance, in the interpolation setting, calculating the RKHS norm of $\bar{s}$ requires computing the inverse of the block operator-valued matrix $K_{XX}$ as well as evaluating inner products in $\mathcal Y^m$, which generally do not have an explicit expression. Furthermore, although the bound in Theorem~\ref{theorem_1} has an analytical form, its evaluation still requires solving an optimization problem over a potentially infinite-dimensional space, as defined in \eqref{eq_delta_1} and \eqref{eq_delta_2}. 

Unlike the scalar-valued case, for vector-valued kernels, the computation of quantities such as inner products and norms can be in infinite-dimensional Hilbert spaces, which do not have closed-form solutions with arbitrary kernels. In what follows, we restrict our attention to separable kernels. Specifically, we assume that
\[K(s,t) = G(s,t)T, \quad \forall s, t \in \mathcal{X},
\]
where $G:\mathcal{X}\times\mathcal{X}\rightarrow\mathbb{R}$ is a scalar-valued positive definite kernel, and $T\in\mathcal{L}_{+}(\mathcal{Y})$ is a positive linear operator.

\begin{remark}
    Assuming a separable kernel is a standard approach for infinite-dimensional learning problems \cite{li2024towards}. Although this assumption excludes certain classes of operator-valued kernels, it still encompasses a broad and practically relevant family, e.g., the diagonal kernel. Such kernels are commonly found in the literature, both in theoretical analyses \cite{kadri2016operator,li2024towards} and in practical applications \cite{brogat2022vector,yang2025kernel}.
\end{remark}

Let the eigendecomposition of the scalar kernel matrix be
\[
G_{XX}
=
\sum_{i=1}^{m}
\lambda_i^G\,\theta_i\theta_i^{\top},
\]
where $G_{XX}\in\mathbb{R}^{m\times m}$ is the finite-dimensional kernel matrix with $(G_{XX})_{ij} = G(x_i,x_j)\in \mathbb{R}$, $\{\lambda_i^G\}_{i=1}^m$ are its eigenvalues and $\{\theta_i\}_{i=1}^m$ are the corresponding eigenvectors. 

We assume that there exists an orthonormal basis of eigenfunctions $\{\phi_j\in \mathcal{Y}, j\geq1\}$ associated with eigenvalues $\{\lambda_j^T\in\mathbb{R}, j\geq1\}$ \cite{kadri2016operator} such that
\[
T = \sum_{j} \lambda_j^T\phi_j\phi_j^*.
\]
When $\mathcal{Y}$ is a finite-dimensional space, e.g., $\mathbb{R}^n$, the operator $T$ admits a finite-dimensional matrix representation. If $\mathcal Y$ is infinite-dimensional (e.g.\ a Sobolev space or $L^2$ space), then $T$ admits a countable spectral expansion. In practice, we truncate this expansion at level $n$, yielding the finite-rank approximation $T_n$, which acts on the finite-dimensional subspace
$\operatorname{span}\{\phi_j : j\in[n]\}\subset \mathcal Y$. We denote the diagonal matrix whose diagonal entries are the eigenvalues of $T_n$ by $\Lambda_{T_n}$, i.e.,
\[
\Lambda_{T_n} = \operatorname{diag}(\lambda_1^T,\dots,\lambda_n^T).
\]

Under the separable kernel assumption, the block operator matrix $K_{XX}$ admits a Kronecker representation
\[
K_{XX} = G_{XX}\otimes T,
\]
where $\otimes$ denotes the Kronecker product. Moreover, we write $K_{Xx}=G_{Xx}\otimes T$ and $K_{xX}=G_{xX}\otimes T$ with $G_{Xx}\in\mathbb{R}^{m\times1}$ and $G_{xX}\in\mathbb{R}^{1\times m}$, respectively. When $T$ is approximated by the finite-rank operator $T_n$, Assumption~\ref{assumption_4} is automatically satisfied provided $G_{XX}$ and $T_n$ are invertible, since $K_{XX}^{-1} = G_{XX}^{-1}\otimes T_n^{-1}$.

The eigenpairs of $(K_{XX}+\lambda I)^{-1}$ are given by
\[
\big(\theta_i\otimes\phi_j,\;
(\lambda_i^G\lambda_j^T+\lambda)^{-1}\big).
\]
Here, $\theta_i\otimes\phi_j$ is an eigenfunction of $K_{XX}+\lambda I$, and
$(\lambda_i^G\lambda_j^T+\lambda)^{-1}$ is the corresponding eigenvalue of its inverse. As a result, we can represent $(K_{XX}+\lambda I)^{-1}$ via its spectrum
\begin{equation}
\label{eq_spectrum}
(K_{XX}\!+\!\lambda I)^{-1}
\!=\!
\sum_{i=1}^{m}
\sum_{j=1}^{n}
(\lambda_i^G\lambda_j^T\!+\!\lambda)^{-1}
(\theta_i\otimes\phi_j)
(\theta_i\otimes\phi_j)^*.
\end{equation}

The coefficient vector $\boldsymbol{\alpha}^*$ and the observation vector $\boldsymbol{y}$ can be represented by finite coordinate matrices $A \in \mathbb R^{m\times n}$ and $Y \in \mathbb R^{m\times n}$ such that
\[
\alpha_i^* = \sum_{j=1}^{n} A_{ij}\,\phi_j,
\qquad
y_i = \sum_{j=1}^{n} Y_{ij}\,\phi_j,
\quad \forall\, i \in [m].
\]
% \begin{remark}
%     When $\mathcal{Y}$ is infinite dimensional, with $T$ approximated by $T_n$, only the projection of elements in $\mathcal Y$ onto the subspace $\mathcal Y_n$ is relevant. Each element of $\mathcal Y_n$ admits a finite-dimensional representation under the orthonormal basis $\{\phi_j\}_{j=1}^n$.
% \end{remark}

With the spectrum representation \eqref{eq_spectrum}, the coordinate matrix $A$ can be efficiently calculated via
\begin{align*}
    A_{ij}= \sum_{k = 1}^m(\lambda_k^G\lambda_j^T + \lambda)^{-1}\theta_k(i)\theta_k^{\top} Y_{:,j},
\end{align*}
where $Y_{:,j}$ is the $j$-th column of matrix $Y$.

% \begin{remark}
% When the output space is finite-dimensional, such as $\mathbb{R}^n$, the operator $T$ admits a matrix representation. In this case, quantities such as $\bm{\alpha}^*$ can be computed via standard matrix--vector operations in $\mathbb{R}^{mn}$.
% However, this is computationally inefficient, since it requires directly inverting a matrix in $\mathbb{R}^{mn \times mn}$, which becomes prohibitive for large $m$ or $n$. In contrast, a spectral representation of $T$ explicitly reveals the structure of the output space, enabling efficient computation of the inverse by decoupling the problem along the eigendirections. This leads to significant computational savings and a clearer interpretation of the operator action.
% \end{remark}

Following the same spectral decomposition argument, all quantities appearing in Theorem~\ref{theorem_1} admit explicit finite-dimensional representations under the separable-kernel assumption. 

First, the operator norm of $P^{\frac{1}{2}}(x)$ reduces to
\[
\|P^{\frac{1}{2}}(x)\|
=
\sqrt{G(x,x)-G_{xX}G_{XX}^{-1}G_{Xx}}\sqrt{\lambda_{\max}^T},
\]
where $\lambda_{\max}^T := \max_{j\in[n]} \lambda_j^T$. The RKHS norm of the noisy interpolant satisfies
\[
\|\hat{s}\|_{\mathcal H}^2
=
\operatorname{tr}(G_{XX}^{-1}Y\Lambda_{T_n}^{-1}Y^{\top}).
\]

Moreover,

\begin{align*}
    \Big\|K_{xX}\big((K_{XX}+\lambda I)^{-1}-K_{XX}^{-1}\big)\bm{y}\Big\|_{\mathcal{Y}}
    =\|G_{xX}\Theta\epsilon\Lambda_{T_n}\|_2,
\end{align*}
where $\Theta$ is the matrix with columns consisting of $\theta_i$, $\epsilon$ is the coordinate matrix of $\big((K_{XX}+\lambda I)^{-1}-K_{XX}^{-1}\big)\bm{y}$ under the basis $\theta_i\otimes \phi_j$. Its elements are given by
\[
\epsilon_{ij} = \Big ((\lambda_{i}^G\lambda_{j}^T + \lambda)^{-1}-(\lambda_{i}^G\lambda_{j}^T)^{-1}\Big)\theta_i^{\top}Y_{:,j}.
\]

The optimization problem~\eqref{eq_delta_1} reduce to finite-dimensional programs. Let $\Omega\in\mathbb R^{m\times n}$ denote the coordinate matrix of
$\boldsymbol{\delta}$ under the basis $\{\phi_j\}_{j=1}^n$, i.e., $\delta_i=\sum_{j=1}^{n}\Omega_{ij}\phi_j$.
Then problem~\eqref{eq_delta_1} becomes
\begin{align*}
    \max_{\Omega\in\mathbb{R}^{m\times n}}\quad&2\operatorname{tr}(G_{XX}^{-1}Y\Lambda_{T_n}^{-1}\Omega^{\top})-  \operatorname{tr}(G_{XX}^{-1}\Omega\Lambda_{T_n}^{-1}\Omega^{\top}),\\
        \text{s.t.}\quad&\|\Omega_{i,:}\|_{2}\leq \bar{\delta},\quad \forall i \in [m],
\end{align*}
where $\Omega_{i,:}$ denotes the $i$-th row of $\Omega$.

Problem \eqref{eq_delta_2} admits an explicit upper bound $\|G_{xX}G_{XX}^{-1}\|_1\bar{\delta}$ since
\[\|K_{xX}K_{XX}^{-1}\bm{\delta}\|_{\mathcal{Y}} = \|G_{xX}G_{XX}^{-1}\otimes I \bm{\delta}\|_{\mathcal{Y}}\leq\|G_{xX}G_{XX}^{-1}\|_1\bar{\delta}.
\]


% \begin{remark}
%     Note that when the output space $\mathcal Y$ is infinite-dimensional, approximating the operator $T$ by a finite-dimensional spectral expansion induces an approximation of the bound in Theorem~\ref{theorem_1}. Such an approximation effectively restricts the hypothesis class to operators mapping from the input space $\mathcal X$ into a finite-dimensional subspace $\mathcal Y_n \subset \mathcal Y$. As a consequence, the resulting bound measures the discrepancy between $s^*(x)$ and the projection of $f(x)$ onto $\mathcal Y_n$, which is necessarily no larger than the true upper bound. Indeed, for any $f(x) \in \mathcal Y$, one can write the orthogonal decomposition $f(x) = v + w$, where $v \in \mathcal Y_n, \; w \in \mathcal Y_n^\perp$. Then, $ \|s^*(x) - f(x) \|_{\mathcal Y}\le\| s^*(x) - v \|_{\mathcal Y} + \| w \|_{\mathcal Y}$. Here, only the first term is controlled by the finite-dimensional bound, while the second term represents the approximation error introduced by truncating the spectral expansion.
% \end{remark}

